Modelling the Near-IR Spectra of Red Supergiant-dominated Populations

We report on recent progress in the modelling of the near-IR spectra of young stellar populations, i.e. populations in which red supergiants (RSGs) are dominant. First, we discuss the determination of fundamental parameters of RSGs using fits to their near-IR spectra with new PHOENIX model spectra; RSG-specific surface abundances are accounted for and effects of the microturbulence parameter are explored. New population synthesis predictions are then described and, as an example, it is shown that the spectra of young star clusters in M82 can be reproduced very well from 0.5 to 2.4 micrometers. We warn of remaining uncertainties in cluster ages.

==> sissa_abstract <==
Title:  Modelling the Near-IR Spectra of Red Supergiant-dominated Populations
Authors: A. Lan\c{c}on, J.S. Gallagher, R. de Grijs, P. Hauschildt,
  D. Ladjal, M. Mouhcine, L.J. Smith, P.R. Wood, N. F\"orster Schreiber
Comments: Proceedings of IAU Symp. 241 on Stellar Populations as Building
  Blocks of Galaxies, ed. A. Vazdekis et al. (2007). 4 pages, 6
  postscript figures, uses iaus.cls.

 We report on recent progress in the modelling of the near-IR spectra of young
stellar populations, i.e. populations in which red supergiants (RSGs) are
dominant. First, we discuss the determination of fundamental parameters
of RSGs using fits to their near-IR spectra with new PHOENIX model spectra; 
RSG-specific surface abundances are accounted for and effects of the
microturbulence parameter are explored. New population synthesis predictions 
are then described and, as an example, it is shown that the spectra of young
star clusters in M82 can be reproduced very well from 0.5 to 2.4 micrometers.
We warn of remaining uncertainties in cluster ages.

